Theory of Capillary Tension and Interfacial Dynamics of Motility-Induced Phases

The statistical mechanics of equilibrium interfaces has been well-established for over a half century. In the last decade, a wealth of observations have made increasingly clear that a new perspective is required to describe interfaces arbitrarily far from equilibrium. In this work, beginning from microscopic particle dynamics that break time-reversal symmetry, we systematically derive the interfacial dynamics of coexisting motility-induced phases. Doing so allows us to identify the athermal energy scale that excites interfacial fluctuations and the nonequilibrium surface tension that resists these excitations. Our theory identifies that, in contrast to equilibrium fluids, this active surface tension contains contributions arising from nonconservative forces which act to suppress interfacial fluctuations and, crucially, is distinct from the mechanical surface tension of Kirkwood and Buff. We find that the interfacial stiffness scales linearly with the intrinsic persistence length of the constituent active particle trajectories, in agreement with simulation data. We demonstrate that at wavelengths much larger than the persistence length, the interface obeys surface area minimizing Boltzmann statistics with our derived nonequilibrium interfacial stiffness playing an identical role to that of equilibrium systems.

==> custom-commands.tex <==
\usepackage{multirow}

% ******** CUSTOMIZATIONS  ******** %
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

%******** FONT FORMATTING ********%
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}

\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
%new command
\newcommand{\xmark}{\ding{55}}%
\newcommand*\diff{\mathop{}\!\mathrm{d}}

%When editing
%\newcommand{\ed}[1]{{\color{blue}#1}}
\newcommand{\ed}[1]{{\color{black}#1}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}

\makeatletter
\DeclareRobustCommand{\svdots}{%
  \hbox{ }\vbox{%
    \baselineskip 3\p@
    \lineskiplimit \z@
    \kern 1\p@
    \hbox{.}\hbox{.}\hbox{.}%
  }%
  \hbox{ }
}
\makeatother

\makeatletter
\def\overvect@#1#2#3{\vbox{\ialign{##\crcr
       \noalign{\kern-.7pt\nointerlineskip}#1#2\crcr
       \noalign{\kern1pt\nointerlineskip}$\m@th\hfil#2#3\hfil$\crcr}}}
\makeatother
\def\*#1{\mathbf{#1}}
%\newcommand{\todo}[1]{\textcolor{RedViolet}{[ToDo: #1]}}
\newcommand{\fvect}[1]{\overset{\rightarrow}{#1}}
\newcommand{\bvect}[1]{\overset{\leftarrow}{#1}}
\newcommand{\scp}{\mathcal{P}}
\newcommand{\bscp}{\partial \scp}

\DeclareMathOperator\erfc{erfc}
% increase line spacing in matrix environments
\makeatletter
\renewcommand*\env@matrix[1][\arraystretch]{%
  \edef\arraystretch{#1}%
  \hskip -\arraycolsep
  \let\@ifnextchar\new@ifnextchar
  \array{*\c@MaxMatrixCols c}}
\makeatother

% better circled text
\newcommand*\circled[1]{
	\tikz[baseline=(char.base)]{
		\node[shape=circle,draw,inner sep=1pt] (char) {#1};
	}
}
%coloring in math mode
\makeatletter
\def\mathcolor#1#{\@mathcolor{#1}}
\def\@mathcolor#1#2#3{%
  \protect\leavevmode
  \begingroup
    \color#1{#2}#3%
  \endgroup
}
\makeatother

%short arrow that can rotate
\makeatletter
\newcommand{\fixed@sra}{$\vrule height 2\fontdimen22\textfont2 width 0pt\shortrightarrow$}
\newcommand{\shortarrow}[1]{%
  \mathrel{\text{\rotatebox[origin=c]{\numexpr#1*45}{\fixed@sra}}}
}
\makeatother
\makeatletter
\newcommand{\blankarrow}{\textcolor{white}{\shortarrow{1}}}
\makeatother

%boxing characters
\makeatletter
\renewcommand{\boxed}[1]{\text{\fboxsep=.2em\fbox{\m@th$\displaystyle#1$}}}
\makeatother

%small fraction
\newcommand\ddfrac[2]{\frac{\displaystyle #1}{\displaystyle #2}}
%\geometry{margin=1in}

%short to
\newcommand{\shortto}[1][3pt]{\mathrel{%
   \hbox{\rule[\dimexpr\fontdimen22\textfont2-.2pt\relax]{#1}{.4pt}}%
   \mkern-4mu\hbox{\usefont{U}{lasy}{m}{n}\symbol{41}}}}

\def\doubleunderline#1{\underline{\underline{#1}}}

%TikZ code "illustrating" the new "brace"
\newcommand{\newbrace}[1][]{
\begin{tikzpicture}[baseline=-0.5ex]
\draw[#1] (0,0) -- (0.3,0.3);
\draw[#1] (0,0) -- (0.3,-0.3);
\end{tikzpicture}
}

% the optional argument allows you to select the type of arrow 
% you can also customize the "new brace"
\newenvironment{casesnew}[1][->]%
{\;\newbrace[#1]\;\begin{array}{@{}l@{}}}%
{\end{array}}

%Declaring some math operators
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\sech}{sech}
\allowdisplaybreaks

\renewcommand{\thefigure}{S.\arabic{figure}}
\renewcommand{\thetable}{S.\arabic{table}}

\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\DontPrintSemicolon
% Define pseudocode formatting
\renewcommand{\KwSty}[1]{\textnormal{\textcolor{blue!90!black}{\ttfamily\bfseries #1}}\unskip}
\renewcommand{\ArgSty}[1]{\textnormal{\ttfamily #1}\unskip}
\SetKwComment{Comment}{\color{green!50!black}// }{}
\renewcommand{\CommentSty}[1]{\textnormal{\ttfamily\color{green!50!black}#1}\unskip}
\newcommand{\assign}{\leftarrow}
\newcommand{\var}{\texttt}
\newcommand{\FuncCall}[2]{\texttt{\bfseries #1(#2)}}
\SetKwProg{Function}{function}{}{}
\renewcommand{\ProgSty}[1]{\texttt{\bfseries #1}}


%%%%%%%%%%%%%%%%%%%%%%% Wide tilde %%%%%%%%%%%%
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{stackengine}
\usepackage{scalerel}
